Data-Driven Probabilistic Fault Detection and Identification via Density Flow Matching

Fault detection and identification (FDI) is critical for maintaining the safety and reliability of systems subject to actuator and sensor faults. In this paper, the problem of FDI for nonlinear control-affine systems under simultaneous actuator and sensor faults is studied. We model fault signatures through the evolution of the probability density flow along the trajectory and characterize detectability using the 2-Wasserstein metric. In order to introduce quantifiable guarantees for fault detectability based on system parameters and fault magnitudes, we derive upper bounds on the distributional separation between nominal and faulty dynamics. The latter is achieved through a stochastic contraction analysis of probability distributions in the 2-Wasserstein metric. A data-driven FDI method is developed by means of a conditional flow-matching scheme that learns neural vector fields governing density propagation under different fault profiles. To generalize the data-driven FDI method across continuous fault magnitudes, Gaussian bridge interpolation and Feature-wise Linear Modulation (FiLM) conditioning are incorporated. The effectiveness of our proposed method is illustrated on a spacecraft attitude control system, and its performance is compared with an augmented Extended Kalman Filter (EKF) baseline. The results confirm that trajectory-based distributional analysis provides improved discrimination between fault scenarios and enables reliable data-driven FDI with a lower false alarm rate compared with the augmented EKF.

==> introduction.tex <==
\section{Preliminaries}
\subsection{Continuous Time Deterministic Systems}
Consider the following continuous-time nonlinear system and its virtual dynamics
\begin{equation}
\label{eq:system_ode}
\dot{\xb}=\fb(\xb(t)), \quad \delta \dot{\xb}=\frac{\partial \fb(\xb, t)}{\partial \xb} \delta \xb
\end{equation}
where $\fb:\mathscr{X} \to \mathscr{X}$ is a smooth vector field, $\xb \in \mathscr{X}$ is the state, and $\delta \xb \in \mathscr{T}_{\xb} \mathscr{X}$ is the virtual displacement. Together they form the \emph{prolonged system} which is a smooth vector field on the tangent bundle $(\xb, \delta \xb) \in \mathscr{T} \mathscr{X}$. Let $\Phi:\mathscr{X} \times \R \to \mathscr{X}$ be the flow map of~\eqref{eq:system_ode} i.e. $\Phi_t(\xb_0):=\Phi(\xb_0,t)$ is a solution to~\eqref{eq:system_ode} with initial condition $\xb(0) = \xb_0$.  
\subsection{Perron-Frobenius Operator}
The Perron-Frobenius operator (PFO) $\mathcal{P}^t: L^1(\mathscr{X})\to L^1(\mathscr{X})$ associated with the flow map $\Phi_t$ is defnined as
\begin{equation}
\int_{\mathbb{A}}\left[\mathcal{P}^t \rho\right](x) d x=\int_{\left(\Phi^t\right)^{-1}(\mathbb{A})} \rho(x) d x
\end{equation}
for any $\mu$-measurable set $\mathbb{A}$, assuming that the relevant measure $\mu$ is absolutely continuous with respect to the Lebesgue measure and can thus be expressed in terms of a density $\rho$ i.e., $d \mu(x)=\mu(d x)=\rho(x) d x$. It can be shown that the family of these operators $\left\{\mathcal{P}^t\right\}_{t \geq 0}$ form a semigroup. The generator of this semigroup is known as the Liouville operator, denoted $\mathcal{L}$, or Perron-Frobenius generator and expresses the defnormation of the density $\rho$ under infinitesimal action of the operator $\mathcal{P}^t$. That is,
\begin{equation*}
\frac{d \rho}{d t}=\mathcal{L} \rho=-\nabla_x \cdot(\rho \fb).
\end{equation*}
Alternatively, the action of the generator can be written in terms of the Perron-Frobenius operator as
\begin{equation*}
\mathcal{L} \rho=\lim _{t \rightarrow 0} \frac{\mathcal{P}^t \rho-\rho}{t}=\lim _{t \rightarrow 0}\left(\frac{\mathcal{P}^t-\mathcal{I}}{t}\right) \rho
\end{equation*}
where $\mathcal{I}$ is the identity operator. The evolution of the measure is given by the Liouville equation
\begin{equation*}
    \partial_t \rho_t + \nabla \cdot (\fb \rho_t) = 0, \quad \rho(\mathbf{x}, 0)=\rho_0(\mathbf{x}) \quad \forall \mathbf{x} \in \mathscr{X}.
\end{equation*}
Via the change of variables formula, the evolution of the Liouville equation under dynamics~\eqref{eq:system_ode} is equivalently:
\begin{equation*}
    \frac{d}{d t} \log \rho(\mathbf{x}, t)=-\operatorname{Tr}(\mathbf{J}(\mathbf{x}, t)).
\end{equation*}
Similarly, the PFO has an equivalent form of:
\begin{equation}
    \mathcal{P}^\tau \rho(\mathbf{x})=\rho\left(\Phi(\mathbf{x}, -\tau)\right)\left|\operatorname{det} D_x \Phi(\mathbf{x}, -\tau)\right|
\end{equation}
\begin{equation*}
\mathcal{P}^t \rho(\mathbf{x})=\rho(\Phi_{-t}(\mathbf{x})) \exp\left(-\int_0^t \operatorname{Tr}(\mathbf{J}(\Phi_s(\mathbf{x}), s)) d s\right)
\end{equation*}
where $\mathbf{J}(\mathbf{x}, t)=\frac{\partial \fb(\mathbf{x}, t)}{\partial \mathbf{x}}$ is the Jacobian of the vector field $\fb$.
\begin{lem}[Contraction Theory]
\label{lem:contraction_theory}
The system~\eqref{eq:system_ode} is contracting (i.e., all the solution trajectories exponentially converge to a single trajectory globally from any initial condition), if there exists a uniformly positive defninite metric $M(\xb, t)=\Theta(\xb, t)^T \Theta(\xb, t)$, $M(\xb, t) \succeq \underline{m} I, \forall \xb, t$, with a smooth coordinate transformation of the virtual displacement $\delta \zb=\Theta(\xb, t) \delta \xb$ s.t.
\begin{equation*}
\frac{\partial f^T}{\partial \xb} M(\xb, t)+\dot{M}(\xb, t)+M(\xb, t) \frac{\partial f}{\partial \xb} \preceq-2 \gamma M(\xb, t), \quad \forall \xb, t
\end{equation*}
where $\gamma$ and $\underline{m}$ are some positive constants. If the system (1) is contracting, then the following equation holds
\begin{equation*}
\|\delta \zb(t)\|=\|\Theta(\xb, t) \delta \xb(t)\| \leq\|\delta \zb(0)\| e^{-\gamma t}
\end{equation*}
\begin{pf}
    Put standard contraction results here.
\end{pf}
\end{lem}
\begin{cor}[Equivalent Contraction Conditions]
A function $f:\R^n \to \R^n$ is contracting in the identity metric $M(\xb, t) = I$ if and only if there exists a constant $\beta > 0$ such that 
\begin{equation*}
\frac{\partial f^T}{\partial \xb} + \frac{\partial f}{\partial \xb} \preceq -\beta I, \quad \forall \xb, t
\end{equation*}
which is equivalent to 
\begin{equation*}
    (f(\xb)-f(\yb), \xb-\yb) \leq-\beta\|\xb-\yb\|^2, \quad \forall \xb, \yb \in \R^n
\end{equation*}
\end{cor}
\section{Stochastic Systems}
Consider the Ito stochastic differential equation (SDE)
\begin{equation}
    \label{eq:sde}
\left\{\begin{array}{l}
d \xb_t=f\left(\xb_t, t\right) d t+G\left(\xb_t, t\right) d \mathscr{W}_t \\
\xb(0)=\xb_0 \in \mathbb{R}^d
\end{array}\right.
\end{equation}
where $\mathscr{W}_t$ is the standard d-dimensional Brownian motion. Let $f:\mathbb{R}^d \times \mathbb{R} \to \mathbb{R}^d$ be the drift and $G:\mathbb{R}^d \times \mathbb{R} \to \mathbb{R}^{d \times d}$ be the diffusion term. Assume that $\exists L_f, s_f,>0, \forall t$ such that 
\begin{equation*}
\begin{aligned}
\|f(\xb, t)-f(\yb, t)\|_2 & \leq L_f\|\xb-\yb\| \quad \forall \xb, \yb \in \mathbb{R}^d \\ 
\|f(\xb, t)\|^2 & \leq s_f\left(1+\|\xb\|^2\right)
\end{aligned}
\end{equation*}    
and the diffusion term $G$ has Lipschitz constant $\|G(\xb, t)-G(\yb, t)\|_{\mathrm{F}} \leq L_G\|\xb-\yb\|$. These standard assumptions gurantee the existence and uniqueness of a strong solution to~\eqref{eq:sde}. 
\begin{defn}
The transition density function $p_\tau: \mathscr{X} \times \mathscr{X} \rightarrow \mathbb{R}_{+}$is defnined as [11]
\begin{equation*}
\mathbb{P}\left[x_{t+\tau} \in \mathbb{B} \mid x_t=x\right]=\int_{\mathbb{B}} p_\tau(x, m) d m, \forall \mathbb{B} \in \mathcal{B}(\mathscr{X})
\end{equation*}
\end{defn}
The transition density function is the infinite-dimensional counterpart of the transition matrix entries for a Markov chain. The stochastic PF operator is defnined as:
\begin{defn} 
Let $\rho \in L^1(\mathscr{X})$ be a probability density function. The Perron-Frobenius semigroup of operator $\mathcal{P}^\tau, \tau>$ 0 , is defnined as $\mathcal{P}^\tau: L^1(\mathscr{X}) \rightarrow L^1(\mathscr{X})$, such that
\begin{equation*}
\mathcal{P}^\tau \rho(\cdot)=\int_{\mathscr{X}} p_\tau(m, \cdot) \rho(m) d m
\end{equation*}
\end{defn}
The PF operator $\mathcal{P}^\tau$ as defnined here is also a linear operator and $\mathcal{P}^\tau \rho$ has an infinitesimal generator $-\nabla \cdot(\rho f)+ \frac{1}{2} \nabla^2\left(g^2 \rho\right)$.
\begin{defn}[Infinitesimal Generator]
Let $h: \mathbb{R}^d \times \mathbb{R} \rightarrow \mathbb{R}$ be a Lebesgue-measurable function. The infinitesimal generator of $h$ along~\eqref{eq:sde} is defnined as
\begin{equation*}
\begin{aligned}
\mathcal{L} h\left(\xb_t, t\right)= & \lim _{\delta t \rightarrow 0} \frac{\mathbb{E}_{\mathscr{W}_{\mathbf{t}}}\left[h\left(\xb_{t+\delta t}, t+\delta t\right)\right]-h\left(\xb_t, t\right)}{\delta t} \\
= & \partial_t h\left(\xb_t, t\right)+\nabla h\left(\xb_t, t\right)^{\top} f\left(\xb_t\right) \\
& +\frac{1}{2} \operatorname{Tr}\left\{G\left(\xb_t, t\right) \nabla^2 h\left(\xb_t, t\right) G\left(\xb_t, t\right)^{\top}\right\} .
\end{aligned}
\end{equation*}
\end{defn}
\subsection{Wasserstein Metric}
Let $\mathscr{P}_2(\mathbb{R}^d)$ be the space of probability measures on $\mathbb{R}^d$ with finite second moments. Let $\Gamma(\mu, \nu)$ be the set of the joint probability measures $\pi$ with marginals $\mu$ and $\nu$. The $p$-Wasserstein metric between two measures $\mu, \nu \in \mathscr{P}_2(\mathbb{R}^d)$ is defnined as
\begin{equation*}
\begin{split}
\mathbb{W}_p(\mu, \nu) &= \left( \inf_{\pi \in \Gamma(\mu, \nu)} \int_{\mathbb{R}^d \times \mathbb{R}^d} \|\xb-\yb\|^p \, d\pi(\xb,\yb) \right)^{1/p} \\
&= \left(\inf_{\pi \in \Gamma(\mu, \nu)} \mathbb{E}_{\pi}[\|\xb-\yb\|^p]\right)^{1/p}
\end{split}
\end{equation*} 
such that $(\xb,\yb) \sim \pi \in \Gamma(\mu,\nu)$. 
\subsection{Contraction in Wasserstein Space}
\begin{thm}[Contraction in Wasserstein Space]
\label{thm:contraction_in_wasserstein_space}
Let $\{\xb_t\}_{t \geq 0}$ be the solution to~\eqref{eq:sde} with initial distribution $\mu_0 \in \mathscr{P}_2(\mathbb{R}^d)$. Let $f$ be $\beta$-contracting w.r.t the 2-norm, then if $\beta > L^2_G /2$, then the solution $\mu_t \in \mathscr{P}_2(\mathbb{R}^d)$ of process $\{\xb_t\}_{t \geq 0}$ converges in the 2-Wasserstein metric to a unique stationary measure $\mu^* \in \mathscr{P}_2(\mathbb{R}^d)$.
\end{thm}
\begin{pf}
Let $\{\xb_t(\xb_0, \omega)\}_{t \geq 0}$ and $\{\yb_t(\yb_0, \omega)\}_{t \geq 0}$ both be strong solutions to~\eqref{eq:sde} with different initial conditions $\xb_0,\yb_0 \in \mathbb{R}^d, \xb_0 \neq \yb_0$ and the \emph{same} noise realization $\omega$. Using $h = \|x\|_2^2$ and evaluating the infinitesimal generator on the process $\{\zb_t\}_{t \geq 0} = \{\xb_t - \yb_t\}_{t \geq 0}$, we have:
\begin{equation*}
\begin{split} \mathcal{L} h(\zb) & =\nabla h(\zb) \cdot(f(\xb)-f(\yb)) \\
    +&\frac{1}{2} \operatorname{Tr}\left[(G(\xb, t)-G(\yb, t))(G(\xb, t)-G(\yb, t))^{\top} \nabla^2 h(\zb)\right] \\ & =2(f(\xb)-f(\yb)) \cdot \zb \\
    +&\operatorname{Tr}\left[(G(\xb, t)-G(\yb, t))(G(\xb, t)-G(\yb, t))^{\top}\right] \\ & =2(f(\xb)-f(\yb)) \cdot \zb+\|G(\xb, t)-G(\yb, t)\|_{\mathrm{F}}^2 . 
\end{split}
\end{equation*}
By the contraction property of $f$ and the Lipschitz continuity of $G$, we have:
\begin{equation*}
    \mathcal{L} h(\zb) \leq-2 \beta\|\zb\|^2+L_G^2\|\zb\|^2=-\left(2 \beta-L_G^2\right) h(\zb).
\end{equation*}
Using Dynkin's formula $\frac{d}{d t} \mathbb{E}\left[h\left(\zb_t\right)\right]=\mathbb{E}\left[\mathcal{L} h\left(\zb_t\right)\right]$ and applying Gronwall's inequality, we obtain:
\begin{equation*}
    \mathbb{E}\left[h\left(\zb_{t}\right)\right] \leq \mathbb{E}\left[h\left(\zb_{0}\right)\right] e^{-(2\beta - L^2_G)t}.
\end{equation*}
Let $\mu_t \in \mathscr{P}_2\left(\mathbb{R}^d\right)$ be the probability measure associated to the process $\left\{\xb_t\right\}_{t \geq 0}$ and $\nu_t \in \mathscr{P}_2\left(\mathbb{R}^d\right)$ be the probability measure associated to the process $\left\{\yb_t\right\}_{t \geq 0}$. Let now $\Gamma_t$ denote the set of joint probability measures $\pi_t$ having marginals $\mu_t$ and $\nu_t$. Taking the expectation w.r.t the joint measure $\pi_t \in \Gamma_t$ we know that:
\begin{equation*}
    \mathbb{W}_2^2\left(\mu_t, \nu_t\right) \leq \mathbb{E}_{\pi_t}\left[h\left(\zb_t\right)\right] \leq \mathbb{E}_{\pi_0}\left[h\left(\zb_0\right)\right] e^{-(2\beta - L^2_G)t}
\end{equation*}
since the infimum over all couplings $\pi_t$ lower bounds one admissible coupling $\pi_t$ given by the joint distribution of the two processes $\{\xb_t, \yb_t\}$. Minimizing w.r.t $\pi_0$ gives:
\begin{equation*}
\inf _{\pi_0 \in \Gamma_0} \mathbb{E}_{\pi_t}\left[h\left(\zb_t\right)\right] \leq \mathbb{W}_2^2\left(\mu_0, \nu_0\right) e^{-\left(2 \beta-L^2_G\right) t}.
\end{equation*}
By the optimality of the infimum w.r.t the joint measure $\pi_t \in \Gamma_t$, we have:
\begin{equation*}
    \mathbb{W}_2^2\left(\mu_t, \nu_t\right) \leq \mathbb{W}_2^2\left(\mu_0, \nu_0\right) e^{-\left(2\beta - L^2_G\right)t}.
\end{equation*}
\end{pf}
Moreover, observe that if we have instead the stochastic differential equation driven by a homogenous noise term, then there would be no discounting factor of the contractivity of the drift. 
\begin{lem}[Uniqueness in Law]
\label{lem:uniqueness_in_law}    
The uniqueness of a strong solution to~\eqref{eq:sde} for any fixed $\xb_0$ implies pathwise uniqueness defnined by defn 2 of~\cite{yamada1971uniqueness} which implies uniqueness in law defnined by Proposition 1 of~\cite{yamada1971uniqueness}. Moreover, for any fixed $t\geq 0$ the map $F: \mathscr{P}_2(\mathbb{R}^d) \to \mathscr{P}_2(\mathbb{R}^d)$ with $\mu \mapsto \mu_t:= Law(\xb_t)$ where $\xb_t$ is the solution to~\eqref{eq:sde} with initial distribution $\xb_0 \sim \mu$ is well defnined~\cite{yamada1971uniqueness} Corollary 2.
\end{lem}
\begin{thm}[Convergence to Stationary Distribution]
\label{thm:convergence_to_stationary_distribution}
There exists a unique stationary distribution $\mu_{\infty} \in \mathscr{P}_2\left(\mathbb{R}^d\right)$ such that for any initial distribution $\mu_0 \in \mathscr{P}_2\left(\mathbb{R}^d\right)$ the family $\left(\mu_t\right)_{t \geq 0}$ satisfies $\mathbb{W}_2^2\left(\mu_t, \mu_{\infty}\right) \leq \mathbb{W}_2^2\left(\mu_0, \mu_{\infty}\right)e^{-(2\beta - L^2_G)t}$.
\end{thm}
\begin{pf}
To prove existence, first let $\varphi_T: \mathscr{P}_2\left(\mathbb{R}^d\right) \to \mathscr{P}_2\left(\mathbb{R}^d\right)$ for $t >0$ defined by lem~\ref{lem:uniqueness_in_law}. By thm~\ref{thm:contraction_in_wasserstein_space}, $\varphi_t$ is a contraction w.r.t $\mathbb{W}_2$. Since $(\mathscr{P}_2(\mathbb{R}^d), \mathbb{W}_2)$ is a complete metric space, by application of Banach's fixed point thm, there exists a unique fixed point $\mu^*_{t} \in \mathscr{P}_2\left(\mathbb{R}^d\right)$. For any two $t_1, t_2$, denote by
\begin{equation*}
    \mu^*_{t_1} = \varphi_{t_1}(\mu^*_{t_1}), \quad \mu^*_{t_2} = \varphi_{t_2}(\mu^*_{t_2})
\end{equation*}
the unique Banach fixed points of $\varphi_{t_1}$ and $\varphi_{t_2}$ respectively. Then, $\varphi_{t_1}(\varphi_{t_2}(\mu^*_{t_2})) = \varphi_{t_2}(\varphi_{t_1}(\mu^*_{t_1})) = \varphi_{t_2}(\mu^*_{t_1})$ and so $\varphi_{t_2}(\mu^*_{t_1})$ is a fixed point of $\varphi_{t_1}$. From the uniqueness of the fixed point $\varphi_{t_2}(\mu^*_{t_1}) = \mu^*_{t_1}$, $\mu^*_{t_1}$ is a fixed point of $\varphi_{t_2}$. Thus $\mu^*_{t_1} = \mu^*_{t_2}$. Therefore, there exists exactly one measure $\mu_\infty$ that is a fixed point for all $\varphi_t$ for $t \geq 0$ and thus a stationary measure. Exponential convergence to the stationary distribution from any initial distribution $\mu_0$ follows from the contraction property of~\eqref{eq:sde} in thm~\ref{thm:contraction_in_wasserstein_space}. 
\end{pf}

